Locally Coherent, Globally Incoherent: Bounding Compositional Incoherence in Multi-Component LLM Agents

Multi-component LLM agents assemble probabilistic claims from components that each see only part of a joint problem; the composition can violate basic probability axioms even when every component is locally coherent. We formalise this locally coherent, globally incoherent failure via the compositional residual eps*, the L2 distance from the composed quote to the joint coherent polytope, computable at runtime from system output and the declared cross-component coupling constraints. A product-structure dichotomy characterises when local coherence suffices, and a Rayleigh-quotient prediction matches the observed residual within 7% on three of four relation classes. A hierarchical Boyle-Dykstra projection repairs the composition deterministically; an anytime-valid e-process gives sequential coherence monitoring. Across 1,876 ensemble cliques on a four-LLM mid-tier panel (frontier-panel rerun in Section 5.5), eps* > 0 on 33-94% of cliques, translating to +0.115 nats per bet of regret on 1,770 resolved bets under the proportional allocation rule (the gain collapses to +0.006 under bettors that themselves coherentise). Three intuitive LLM-side mitigations(retrieval, partition-aware prompting, aggregator-LLM) each fail or regress.

==> figures/disagreement_spearman_table.tex <==
\begin{tabular}{@{}lcccc@{}}
\toprule
Relation           & $n_{\eps>0}$ & $\rho(\text{bound}, \eps^\star)$ & $\rho(\text{pair}, \eps^\star)$ & $R^2(\text{pair}, \eps^\star)$ \\
\midrule
\textsc{Neg}       & $343$        & $0.97$ & $0.51$ & $0.29$ \\
\textsc{Partition} & $148$        & $0.83$ & $0.31$ & $0.09$ \\
\textsc{Or}        & $215$        & $0.79$ & $0.49$ & $0.26$ \\
\textsc{And}       & $188$        & $0.70$ & $0.28$ & $0.08$ \\
\bottomrule
\end{tabular}

